BIAS-ID: A Framework for Analyzing Transformation Biases in AI-Generated Image Detectors

Given the surge of harmful AI-generated imagery online, reliably distinguishing authentic images from generated ones has become an urgent research topic. While many proposed detection methods demonstrate high accuracy in controlled settings, their performance often degrades substantially when tested on real-world data. A potential root cause is subtle bias in the detectors' training data. As a result, detectors may rely on spurious correlations instead of learning true forensic artifacts. While recent studies have identified this problem and developed countermeasures, there is not yet an established protocol to evaluate how biased a detector actually is. In this work, we therefore take a step back: First, we discuss what it means for a detector to be biased, and how this differs from a lack of robustness. Second, we propose BIAS-ID, a transparent framework for analyzing and quantifying the presence of transformation biases in AI-generated image detectors. We validate our framework by evaluating six detectors across two datasets, revealing that several state-of-the-art detection methods are strongly affected by common, processing-related biases. Our results highlight the importance of bias-aware evaluation for developing reliable AI-generated image detectors. We provide an easy-to-use library and code to reproduce our results at https://github.com/jonasricker/biasid.

==> assets/figures/ats_header_synthbuster_original.tex <==
\begin{tabular}{@{\ }l@{\hspace{5pt}}r@{\;}cr@{\;}cr@{\;}cr@{\;}rr@{\;}cr@{\;}cr@{\;}cr@{\;}r@{\ }}
\toprule
 & \multicolumn{8}{c}{RAISE-1k (resized)\,/\,Synthbuster} & \multicolumn{8}{c}{RAISE-1k (original)\,/\,Synthbuster} \\
 \cmidrule(l{0pt}r{2pt}){2-9} \cmidrule(l{1pt}r{1pt}){10-17}
 & \multicolumn{2}{c}{$\text{ATS}(X_R)$} & \multicolumn{2}{c}{$\text{ATS}(X_F)$} & \multicolumn{2}{c}{$\text{ATS}(X_R, X_F)$} & $\Delta\text{Acc.}$ & $\Delta\text{AUC}$ & \multicolumn{2}{c}{$\text{ATS}(X_R)$} & \multicolumn{2}{c}{$\text{ATS}(X_F)$} & \multicolumn{2}{c}{$\text{ATS}(X_R, X_F)$} & $\Delta\text{Acc.}$ & $\Delta\text{AUC}$ \\
\midrule


==> assets/figures/ats_header_synthbuster_synthclic.tex <==
\begin{tabular}{@{\ }l@{\hspace{5pt}}r@{\;}cr@{\;}cr@{\;}cr@{\;}rr@{\;}cr@{\;}cr@{\;}cr@{\;}r@{\ }}
\toprule
 & \multicolumn{8}{c}{RAISE-1k\,/\,Synthbuster} & \multicolumn{8}{c}{CLIC2020\,/\,SynthCLIC} \\
 \cmidrule(l{0pt}r{2pt}){2-9} \cmidrule(l{1pt}r{1pt}){10-17}
 & \multicolumn{2}{c}{$\text{ATS}(X_R)$} & \multicolumn{2}{c}{$\text{ATS}(X_F)$} & \multicolumn{2}{c}{$\text{ATS}(X_R, X_F)$} & $\Delta\text{Acc.}$ & $\Delta\text{AUC}$ & \multicolumn{2}{c}{$\text{ATS}(X_R)$} & \multicolumn{2}{c}{$\text{ATS}(X_F)$} & \multicolumn{2}{c}{$\text{ATS}(X_R, X_F)$} & $\Delta\text{Acc.}$ & $\Delta\text{AUC}$ \\
\midrule


==> assets/figures/ats_tables/raise_resized_original_downscaling_bilinear.tex <==
\input{assets/figures/ats_header_synthbuster_original}%
UnivFD & -0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.01)} & -0.143 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.173 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.17, 0.18)} & -0.065 & -0.102 & -0.125 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.14, -0.11)} & -0.143 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.271 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.26, 0.29)} & -0.007 & -0.047 \\
DRCT & 0.093 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.10)} & -0.003 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & 0.091 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.10)} & -0.075 & -0.034 & -0.135 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.14, -0.12)} & -0.003 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & 0.138 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & 0.120 & 0.066 \\
RINE & 0.053 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & -0.122 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.107 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.11)} & -0.102 & -0.065 & -0.107 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.11, -0.10)} & -0.122 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.230 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.24)} & -0.053 & 0.022 \\
AIDE & -0.024 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.01)} & 0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.166 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & 0.021 & 0.094 & -0.028 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.01)} & 0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.168 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.18)} & 0.035 & 0.049 \\
SPAI & 0.049 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.06)} & -0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.114 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.12)} & -0.061 & -0.045 & 0.129 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.14)} & -0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.121 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.13)} & -0.097 & -0.089 \\
B-Free & 0.011 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & -0.124 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.118 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.12)} & -0.067 & -0.037 & -0.077 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.07)} & -0.124 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.201 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.19, 0.21)} & -0.041 & -0.044 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/raise_resized_original_jpeg.tex <==
\input{assets/figures/ats_header_synthbuster_original}%
UnivFD & 0.063 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.07)} & -0.073 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.07)} & 0.151 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.16)} & -0.069 & -0.113 & 0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.03)} & -0.073 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.07)} & 0.159 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.17)} & -0.053 & -0.073 \\
DRCT & 0.218 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.23)} & -0.065 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.184 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.18, 0.19)} & -0.199 & -0.185 & 0.145 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.16)} & -0.065 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.141 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & -0.115 & -0.261 \\
RINE & 0.149 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.14, 0.16)} & -0.148 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.150 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.15)} & -0.139 & -0.112 & 0.010 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.02)} & -0.148 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.213 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.22)} & -0.082 & -0.028 \\
AIDE & -0.547 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.57, -0.52)} & -0.528 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.53, -0.52)} & 1.074 & \textcolor{gray}{\fontsize{5}{5}\selectfont (1.05, 1.10)} & 0.006 & 0.082 & -0.442 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.46, -0.42)} & -0.528 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.53, -0.52)} & 0.970 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.95, 0.99)} & -0.043 & -0.059 \\
SPAI & 0.099 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.12)} & -0.222 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.23, -0.22)} & 0.275 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.27, 0.28)} & -0.165 & -0.132 & -0.065 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.05)} & -0.222 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.23, -0.22)} & 0.303 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.29, 0.32)} & -0.075 & -0.063 \\
B-Free & 0.045 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & -0.093 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.10, -0.09)} & 0.075 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & -0.053 & -0.033 & 0.039 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & -0.093 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.10, -0.09)} & 0.071 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.07)} & -0.046 & -0.059 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/raise_resized_original_upscaling_bilinear.tex <==
\input{assets/figures/ats_header_synthbuster_original}%
UnivFD & 0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.07)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & 0.136 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & 0.009 & -0.016 & 0.058 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.07)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & 0.135 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.12, 0.15)} & 0.005 & 0.030 \\
DRCT & 0.219 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.23)} & 0.010 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & 0.228 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.24)} & -0.170 & -0.076 & -0.027 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.02)} & 0.010 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & 0.058 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & 0.032 & 0.034 \\
RINE & 0.045 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & -0.112 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.12, -0.11)} & 0.158 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.16)} & -0.074 & 0.010 & -0.009 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & -0.112 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.12, -0.11)} & 0.187 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.18, 0.19)} & -0.055 & 0.003 \\
AIDE & -0.289 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.31, -0.27)} & -0.249 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.25, -0.24)} & 0.565 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.55, 0.59)} & 0.024 & 0.056 & -0.109 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.09)} & -0.249 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.25, -0.24)} & 0.425 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.41, 0.44)} & -0.082 & -0.103 \\
SPAI & 0.264 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.24, 0.28)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.08)} & 0.334 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.31, 0.35)} & -0.108 & -0.046 & 0.137 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.12, 0.15)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.08)} & 0.207 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.19, 0.22)} & -0.038 & 0.005 \\
B-Free & 0.008 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & 0.013 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.037 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & 0.010 & 0.001 & 0.036 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & 0.013 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.059 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & 0.004 & 0.007 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_downscaling_bicubic.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & -0.022 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.02)} & -0.144 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.176 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.17, 0.18)} & -0.064 & -0.095 & -0.020 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.02, -0.02)} & -0.032 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.03)} & 0.053 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & -0.006 & -0.059 \\
DRCT & -0.056 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.06, -0.05)} & -0.109 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.11, -0.10)} & 0.165 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & -0.014 & -0.038 & -0.119 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.11)} & -0.123 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.242 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.24, 0.25)} & 0.001 & -0.005 \\
RINE & 0.015 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & -0.176 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.18, -0.17)} & 0.165 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & -0.126 & -0.093 & -0.031 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.03)} & -0.194 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.20, -0.19)} & 0.225 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.23)} & -0.139 & -0.105 \\
AIDE & -0.022 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.01)} & -0.025 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.02)} & 0.161 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.17)} & -0.004 & 0.016 & 0.103 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.09, 0.12)} & -0.088 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.09, -0.08)} & 0.052 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & -0.106 & -0.197 \\
SPAI & -0.004 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.02, 0.01)} & -0.121 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.151 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.14, 0.16)} & -0.064 & -0.047 & -0.035 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.03)} & -0.192 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.20, -0.19)} & 0.232 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.24)} & -0.079 & -0.108 \\
B-Free & 0.006 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.01)} & -0.144 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.138 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.14)} & -0.077 & -0.039 & -0.001 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.00, 0.00)} & -0.225 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.23, -0.22)} & 0.226 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.23)} & -0.116 & -0.143 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_downscaling_bilinear.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & -0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.01)} & -0.143 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.173 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.17, 0.18)} & -0.065 & -0.102 & -0.018 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.02, -0.01)} & -0.033 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.03)} & 0.051 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & -0.007 & -0.066 \\
DRCT & 0.093 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.10)} & -0.003 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & 0.091 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.10)} & -0.075 & -0.034 & -0.027 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.02)} & -0.003 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, 0.00)} & 0.049 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.05)} & 0.017 & 0.030 \\
RINE & 0.053 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & -0.122 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.107 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.11)} & -0.102 & -0.065 & 0.013 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & -0.142 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.130 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.14)} & -0.110 & -0.106 \\
AIDE & -0.024 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.01)} & 0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.166 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & 0.021 & 0.094 & 0.111 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.13)} & -0.075 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.07)} & 0.064 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.07)} & -0.106 & -0.171 \\
SPAI & 0.049 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.06)} & -0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.114 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.12)} & -0.061 & -0.045 & 0.019 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.03)} & -0.128 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.141 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & -0.076 & -0.096 \\
B-Free & 0.011 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & -0.124 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.118 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.12)} & -0.067 & -0.037 & 0.005 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.01)} & -0.214 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.22, -0.21)} & 0.208 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.20, 0.21)} & -0.113 & -0.148 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_grayscale.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & -0.011 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.02, -0.00)} & -0.110 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.12, -0.10)} & 0.124 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.12, 0.13)} & -0.051 & -0.057 & 0.011 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.02)} & 0.005 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.01)} & 0.017 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & -0.004 & -0.042 \\
DRCT & 0.162 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.17)} & -0.050 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.05, -0.05)} & 0.113 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.12)} & -0.156 & -0.118 & -0.041 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.05, -0.03)} & -0.068 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.109 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.12)} & -0.023 & -0.021 \\
RINE & -0.086 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.09, -0.08)} & -0.338 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.34, -0.33)} & 0.424 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.41, 0.43)} & -0.237 & -0.054 & -0.091 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.10, -0.09)} & -0.376 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.38, -0.37)} & 0.467 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.46, 0.48)} & -0.241 & -0.194 \\
AIDE & 0.031 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.02, 0.04)} & 0.009 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & 0.040 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.05)} & -0.011 & -0.041 & 0.060 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.07)} & -0.001 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.00, 0.00)} & 0.059 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.07)} & -0.044 & -0.030 \\
SPAI & -0.124 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.14, -0.11)} & -0.863 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.87, -0.86)} & 0.987 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.97, 1.01)} & -0.380 & -0.271 & -0.288 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.30, -0.27)} & -0.796 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.80, -0.79)} & 1.084 & \textcolor{gray}{\fontsize{5}{5}\selectfont (1.07, 1.10)} & -0.259 & -0.164 \\
B-Free & 0.016 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & -0.010 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.01)} & 0.015 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & -0.003 & -0.001 & 0.007 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.01)} & 0.018 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.02, 0.02)} & 0.026 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.02, 0.03)} & 0.008 & 0.012 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_jpeg.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & 0.063 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.07)} & -0.073 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.07)} & 0.151 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.16)} & -0.069 & -0.113 & 0.084 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.09)} & 0.022 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.02, 0.02)} & 0.119 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.12)} & -0.031 & -0.103 \\
DRCT & 0.218 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.23)} & -0.065 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.184 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.18, 0.19)} & -0.199 & -0.185 & -0.033 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.02)} & -0.042 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.05, -0.04)} & 0.133 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.14)} & -0.005 & -0.003 \\
RINE & 0.149 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.14, 0.16)} & -0.148 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.150 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.15)} & -0.139 & -0.112 & 0.162 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & -0.117 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.12, -0.11)} & 0.128 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.12, 0.13)} & -0.151 & -0.219 \\
AIDE & -0.547 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.57, -0.52)} & -0.528 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.53, -0.52)} & 1.074 & \textcolor{gray}{\fontsize{5}{5}\selectfont (1.05, 1.10)} & 0.006 & 0.082 & -0.364 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.38, -0.35)} & -0.563 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.57, -0.56)} & 0.928 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.91, 0.95)} & -0.114 & -0.166 \\
SPAI & 0.099 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.12)} & -0.222 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.23, -0.22)} & 0.275 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.27, 0.28)} & -0.165 & -0.132 & 0.020 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.03)} & -0.266 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.27, -0.26)} & 0.340 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.33, 0.35)} & -0.143 & -0.172 \\
B-Free & 0.045 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & -0.093 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.10, -0.09)} & 0.075 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & -0.053 & -0.033 & 0.043 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & -0.153 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.16, -0.15)} & 0.119 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.11, 0.12)} & -0.095 & -0.141 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_rotation.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & 0.348 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.33, 0.36)} & 0.287 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.28, 0.30)} & 0.635 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.61, 0.66)} & -0.027 & -0.084 & 0.215 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.23)} & 0.257 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.25, 0.26)} & 0.472 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.46, 0.49)} & 0.021 & 0.012 \\
DRCT & 0.195 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.18, 0.21)} & -0.041 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.04)} & 0.166 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & -0.167 & -0.138 & -0.048 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.05, -0.04)} & -0.058 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.06, -0.05)} & 0.134 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.14)} & -0.010 & -0.006 \\
RINE & 0.267 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.26, 0.28)} & 0.021 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.02, 0.02)} & 0.288 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.28, 0.30)} & -0.144 & -0.098 & 0.133 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.14)} & 0.047 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & 0.180 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.17, 0.19)} & -0.022 & -0.047 \\
AIDE & -0.229 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.25, -0.21)} & -0.147 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.15, -0.14)} & 0.394 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.38, 0.41)} & 0.081 & 0.103 & -0.066 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.05)} & -0.229 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.23, -0.22)} & 0.307 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.29, 0.32)} & -0.081 & -0.157 \\
SPAI & -0.076 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.09, -0.06)} & -0.196 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.20, -0.19)} & 0.274 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.26, 0.29)} & -0.066 & -0.009 & -0.126 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.14, -0.11)} & -0.205 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.21, -0.20)} & 0.335 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.32, 0.35)} & -0.037 & -0.044 \\
B-Free & 0.177 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.17, 0.19)} & -0.064 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.159 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.17)} & -0.104 & -0.052 & 0.062 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.07)} & -0.007 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & 0.141 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.14, 0.15)} & -0.029 & -0.047 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_upscaling_bicubic.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & 0.055 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & 0.082 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.09)} & 0.141 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & 0.018 & -0.005 & 0.077 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & 0.076 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & 0.153 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.16)} & -0.002 & -0.016 \\
DRCT & 0.054 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.06)} & -0.091 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.09, -0.09)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & -0.077 & -0.080 & -0.044 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.05, -0.04)} & -0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.06, -0.06)} & 0.106 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.11)} & -0.004 & -0.027 \\
RINE & 0.013 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & -0.128 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.13, -0.12)} & 0.162 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & -0.081 & 0.001 & -0.000 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, 0.00)} & -0.041 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.04)} & 0.055 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & -0.011 & 0.016 \\
AIDE & -0.373 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.40, -0.35)} & -0.330 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.34, -0.32)} & 0.713 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.69, 0.74)} & 0.024 & 0.059 & -0.251 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.27, -0.23)} & -0.306 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.31, -0.30)} & 0.557 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.54, 0.57)} & -0.021 & -0.072 \\
SPAI & 0.229 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.25)} & 0.074 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & 0.303 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.28, 0.32)} & -0.088 & -0.030 & 0.135 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.12, 0.15)} & 0.142 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.14, 0.15)} & 0.277 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.26, 0.29)} & -0.003 & 0.060 \\
B-Free & -0.000 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.00, 0.00)} & -0.004 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & 0.048 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.05)} & 0.003 & 0.001 & 0.012 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.180 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.18, 0.18)} & 0.194 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.19, 0.20)} & 0.096 & 0.104 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_upscaling_bilinear.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & 0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.07)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & 0.136 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & 0.009 & -0.016 & 0.091 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.08, 0.10)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.07)} & 0.161 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.17)} & -0.011 & -0.048 \\
DRCT & 0.219 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.21, 0.23)} & 0.010 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & 0.228 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.24)} & -0.170 & -0.076 & 0.009 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.02)} & 0.034 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & 0.054 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.06)} & 0.014 & 0.036 \\
RINE & 0.045 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & -0.112 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.12, -0.11)} & 0.158 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.15, 0.16)} & -0.074 & 0.010 & 0.036 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & -0.046 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.05, -0.04)} & 0.045 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.04, 0.05)} & -0.021 & -0.009 \\
AIDE & -0.289 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.31, -0.27)} & -0.249 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.25, -0.24)} & 0.565 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.55, 0.59)} & 0.024 & 0.056 & -0.157 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.17, -0.14)} & -0.217 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.22, -0.21)} & 0.385 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.37, 0.40)} & -0.026 & -0.085 \\
SPAI & 0.264 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.24, 0.28)} & 0.070 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.08)} & 0.334 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.31, 0.35)} & -0.108 & -0.046 & 0.174 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.19)} & 0.140 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.13, 0.15)} & 0.314 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.30, 0.33)} & -0.023 & 0.044 \\
B-Free & 0.008 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.01)} & 0.013 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.01, 0.02)} & 0.037 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & 0.010 & 0.001 & 0.035 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.03, 0.04)} & 0.192 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.19, 0.20)} & 0.227 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.22, 0.23)} & 0.097 & 0.093 \\
\bottomrule
\end{tabular}


==> assets/figures/ats_tables/synthbuster_synthclic_webp.tex <==
\input{assets/figures/ats_header_synthbuster_synthclic}%
UnivFD & -0.024 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.02)} & -0.188 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.19, -0.18)} & 0.213 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.20, 0.22)} & -0.083 & -0.111 & -0.005 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.01, -0.00)} & -0.038 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.04, -0.04)} & 0.050 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.05, 0.05)} & -0.013 & -0.131 \\
DRCT & 0.549 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.54, 0.56)} & 0.125 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.12, 0.13)} & 0.674 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.66, 0.69)} & -0.313 & -0.158 & 0.166 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & 0.167 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.16, 0.17)} & 0.333 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.32, 0.34)} & -0.003 & 0.049 \\
RINE & 0.009 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.00, 0.02)} & -0.401 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.41, -0.40)} & 0.412 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.40, 0.42)} & -0.287 & -0.266 & -0.020 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.03, -0.01)} & -0.382 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.39, -0.38)} & 0.402 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.39, 0.41)} & -0.240 & -0.356 \\
AIDE & -0.515 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.54, -0.49)} & -0.482 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.49, -0.48)} & 0.996 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.97, 1.02)} & 0.025 & 0.063 & -0.320 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.34, -0.30)} & -0.506 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.51, -0.50)} & 0.826 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.81, 0.84)} & -0.104 & -0.172 \\
SPAI & -0.066 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.08, -0.05)} & -0.566 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.57, -0.56)} & 0.649 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.63, 0.66)} & -0.258 & -0.173 & -0.209 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.22, -0.19)} & -0.596 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.60, -0.59)} & 0.814 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.80, 0.83)} & -0.198 & -0.191 \\
B-Free & 0.068 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.07)} & -0.064 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.07, -0.06)} & 0.061 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.06, 0.06)} & -0.045 & -0.026 & 0.074 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.07, 0.08)} & -0.116 & \textcolor{gray}{\fontsize{5}{5}\selectfont (-0.12, -0.11)} & 0.100 & \textcolor{gray}{\fontsize{5}{5}\selectfont (0.10, 0.10)} & -0.089 & -0.133 \\
\bottomrule
\end{tabular}

